Minimization of Ion Micromotion in a Linear Paul Trap with a High Finesse Cavity

We demonstrate minimization of ion micromotion in a linear Paul trap with the use of a high finesse cavity. The excess ion micromotion projected along the optical cavity axis or along the laser propagation direction manifests itself as sideband peaks around the carrier in the ion-cavity emission spectrum. By minimizing the sideband height in the emission spectrum, we are able to reduce the micromotion amplitude to approximately the spread of the ground state wave function. This method is useful for cavity QED experiments as it allows for efficient 3-D micromotion compensation despite optical access limitations imposed by the cavity mirrors. We also show that sub-nanometer micromotion compensation is possible with our current system.

==> tikzlibraryoptikz.code.tex <==
\def\optsetxandyvecbyvalueofkey#1{
  \optsetxvecbyvalueofkey{#1}
  \optsetyvecbyvalueofkey{#1}
}
\def\optsetxvecbyvalueofkey#1{
  \pgfsetxvec{\pgfpoint{\pgfkeysvalueof{#1}}{0pt}}
}
\def\optsetyvecbyvalueofkey#1{
  \pgfsetyvec{\pgfpoint{0pt}{\pgfkeysvalueof{#1}}}
}

% Todo: find out whether this is the right way to introduce keys
% Todo: merge generic height / width with lenses
\pgfkeyssetvalue{/tikz/waist}{0.5cm} % Standard waist
\pgfkeyssetvalue{/tikz/optics diameter}{1cm} % Height of lenses / plates etc
\pgfkeyssetvalue{/tikz/beam splitter width}{0.75 cm} % Height of cubes
\pgfkeyssetvalue{/tikz/flip beam splitter axis}{0} % 1 to flip diagonal 
\pgfkeyssetvalue{/tikz/optical element width}{3cm} % Generic width
\pgfkeyssetvalue{/tikz/optical element height}{1cm} % Generic height
\pgfkeyssetvalue{/tikz/curvature}{1cm} % Generic height


% Define shapes


% Vertical optical elements are vertical on paper (i.e. a vertical
% waveplate), that is the beam passes horizontally through it

% Vertical optical element
\pgfdeclareshape{vertical optical element}{
  \savedanchor{\southwest}{%
    \optsetxvecbyvalueofkey{/tikz/optical element width}
    \optsetyvecbyvalueofkey{/tikz/optical element height}
    \pgfpointxy{-0.5}{-0.5}}
  \savedanchor{\northeast}{%
    \optsetxvecbyvalueofkey{/tikz/optical element width}
    \optsetyvecbyvalueofkey{/tikz/optical element height}
    \pgfpointxy{0.5}{0.5}}
  \savedanchor{\beamnorth}{
    \pgfpointorigin
    \pgf@xa = \pgf@x \pgf@ya=\pgf@y \advance\pgf@ya by
    \pgfkeysvalueof{/tikz/waist}
    \pgfpoint{\pgf@xa}{\pgf@ya}
  }
  
  \anchor{north}{
    % store lower left in xa/ya and upper right in xb/yb 
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y 
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpoint{0}{\pgf@yb}
  }
  \anchor{north west}{
    % store lower left in xa/ya and upper right in xb/yb 
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y 
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpoint{\pgf@xa}{\pgf@yb}
  }
  \anchor{west}{
    % store lower left in xa/ya and upper right in xb/yb 
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y 
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpoint{\pgf@xa}{0}
  }
  \anchor{south west}{\southwest}
  \anchor{south}{
    % store lower left in xa/ya and upper right in xb/yb 
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y 
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpoint{0}{\pgf@ya}
  }
  \anchor{south east}{
    % store lower left in xa/ya and upper right in xb/yb 
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y 
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpoint{\pgf@xb}{\pgf@ya}
  }
  \anchor{east}{
    % store lower left in xa/ya and upper right in xb/yb 
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y 
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpoint{\pgf@xb}{0}
  }
  \anchor{north east}{\northeast}
  \anchor{center}{\pgfpointorigin}

  \anchor{beam north}{\beamnorth}
  
  \anchor{beam north west}{%
    \southwest \pgf@xa=\pgf@x
    \beamnorth \pgf@yc = \pgf@y
    \pgfpointorigin
    \pgf@ya = \pgf@y \advance\pgf@ya by \pgf@yc
    \pgfpoint{\pgf@xa}{\pgf@ya}
  }
  \anchor{beam south west}{%
    \southwest \pgf@xa=\pgf@x
    \beamnorth \pgf@yc = \pgf@y
    \pgfpointorigin
    \pgf@ya = \pgf@y \advance\pgf@ya by -\pgf@yc
    \pgfpoint{\pgf@xa}{\pgf@ya}
  }
  \anchor{beam south}{
    \beamnorth \pgf@ya=-\pgf@y
    \pgfpointorigin \pgf@xa = \pgf@x
    \pgfpoint{\pgf@xa}{\pgf@ya}
  }
  \anchor{beam south east}{%
    \northeast \pgf@xa=\pgf@x
    \beamnorth \pgf@yc = \pgf@y
    \pgfpointorigin
    \pgf@ya = \pgf@y \advance\pgf@ya by -\pgf@yc
    \pgfpoint{\pgf@xa}{\pgf@ya}
  }
  \anchor{beam north east}{
    \northeast \pgf@xa=\pgf@x
    \beamnorth \pgf@yc = \pgf@y
    \pgfpointorigin
    \pgf@ya = \pgf@y \advance\pgf@ya by \pgf@yc
    \pgfpoint{\pgf@xa}{\pgf@ya}
  }
  
  \backgroundpath{
    % No rounded corners 
    \pgfsetcornersarced{\pgfpointorigin}
    \pgfpathrectanglecorners{\northeast}{\southwest}
  }
}

% Vertical wave plate
\tikzset{vertical wave plate/.style={vertical optical element,
    optical element height=\pgfkeysvalueof{/tikz/optics diameter},
    optical element width=0.1*\pgfkeysvalueof{/tikz/optics diameter}}}

% Vertical cavity-----------
\pgfdeclareshape{vertical cavity}{
  \savedanchor{\southwest}{%
    \optsetxvecbyvalueofkey{/tikz/optical element width}
    \optsetyvecbyvalueofkey{/tikz/optical element height}
    \pgfpointxy{-0.5}{-0.5}}
  \savedanchor{\innersouthwest}{%
    \optsetxvecbyvalueofkey{/tikz/optical element width}
    \optsetyvecbyvalueofkey{/tikz/optical element height}
    \pgfpointxy{-0.35}{-0.5}}
  \savedanchor{\northeast}{%
    \optsetxvecbyvalueofkey{/tikz/optical element width}
    \optsetyvecbyvalueofkey{/tikz/optical element height}
    \pgfpointxy{0.5}{0.5}}
  \savedanchor{\innernortheast}{%
    \optsetxvecbyvalueofkey{/tikz/optical element width}
    \optsetyvecbyvalueofkey{/tikz/optical element height}
    \pgfpointxy{0.35}{0.5}}
  \savedanchor{\beamnorth}{
    \pgfpointorigin
    \pgf@xa = \pgf@x \pgf@ya=\pgf@y \advance\pgf@ya by
    \pgfkeysvalueof{/tikz/waist}
    \pgfpoint{\pgf@xa}{\pgf@ya}
  }
  \inheritanchor[from=vertical optical element]{north}
  \inheritanchor[from=vertical optical element]{north west}
  \inheritanchor[from=vertical optical element]{west}
  \inheritanchor[from=vertical optical element]{south west}
  \inheritanchor[from=vertical optical element]{south}
  \inheritanchor[from=vertical optical element]{south east}
  \inheritanchor[from=vertical optical element]{east}
  \inheritanchor[from=vertical optical element]{north east}
  \inheritanchor[from=vertical optical element]{center}
  \inheritanchor[from=vertical optical element]{beam north}
  \inheritanchor[from=vertical optical element]{beam north west}
  \inheritanchor[from=vertical optical element]{beam south west}
  \inheritanchor[from=vertical optical element]{beam south}
  \inheritanchor[from=vertical optical element]{beam south east}
  \inheritanchor[from=vertical optical element]{beam north east}

  \backgroundpath{
    % No rounded corners
    \pgfsetcornersarced{\pgfpointorigin}
    \optsetxvecbyvalueofkey{/tikz/optical element width}
    \optsetyvecbyvalueofkey{/tikz/optical element height}

    % Calculate mirror params
    % Todo make them keys
    \newdimen\curvature
    \pgfextractx{\curvature}{\pgfpointxy{0.75}{0}}
    \newdimen\mirrorheight
    \pgfextracty{\mirrorheight}{\pgfpointxy{0}{1}}
    \def\cavityangle{asin(\mirrorheight/(2*\curvature))}
    
    \pgfpathmoveto{\southwest}
    \pgfpathlineto{\innersouthwest}
    \pgfpatharc{180+\cavityangle}{180-\cavityangle}{\curvature}
    \northeast \pgf@ya = \pgf@y
    \southwest \pgf@xa = \pgf@x
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathclose

    \pgfpathmoveto{\northeast}
    \pgfpathlineto{\innernortheast}
    \pgfpatharc{\cavityangle}{-\cavityangle}{\curvature}
    \northeast \pgf@xa = \pgf@x
    \southwest \pgf@ya = \pgf@y
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathclose

    
  }

}

% Lens
% Todo: Find out how width of lens scales nicely if height is changed
% Todo: make it inherit the nodes from vertical optical element where possible
\pgfdeclareshape{vertical lens}{%
  \savedanchor{\centerpoint}{\pgfpointorigin}
  \savedanchor{\semiminor}{%
    \optsetxandyvecbyvalueofkey{/tikz/optics diameter} \pgfpointxy{0.2}{0}}
  \savedanchor{\semimajor}{%
    \optsetxandyvecbyvalueofkey{/tikz/optics diameter} \pgfpointxy{0}{0.5}}

  \savedanchor{\beamnorth}{%
    \pgfpointorigin
    \pgf@xa = \pgf@x
    \pgf@ya = \pgf@y \advance\pgf@ya by \pgfkeysvalueof{/tikz/waist}
    \pgfpoint{\pgf@xa}{\pgf@ya}}

  \anchor{center}{\centerpoint}    
  \anchor{north}{\semimajor}
  \anchor{east}{\semiminor}
  \anchor{west}{%
    \pgf@process{\semiminor} \pgf@xa = -\pgf@x \pgf@ya=\pgf@y
    \pgfpoint{\pgf@xa}{\pgf@ya}
  }
  \anchor{south}{%
    \pgf@process{\semimajor} \pgf@xa = \pgf@x \pgf@ya =-\pgf@y
    \pgfpoint{\pgf@xa}{\pgf@ya}
  }

  \anchor{beam north}{\beamnorth}
  \anchor{beam south}{
    \beamnorth \pgf@xa=\pgf@x \pgf@ya = -\pgf@y
    \pgfpoint{\pgf@xa}{\pgf@ya}
  }

  \backgroundpath{
    % No rounded corners 
    \pgfsetcornersarced{\pgfpointorigin}
    \semimajor \pgf@xa =\pgf@x \pgf@ya = \pgf@y
    \semiminor \pgf@xb = \pgf@x \pgf@yb = \pgf@y

    % Calculate x and y coordinates of support for bezier curve
    \pgf@xc = \pgf@xb \advance \pgf@xc by 0.1\pgf@xb
    \pgf@yc = 0.5\pgf@ya
    
    % Draw first half of the lens
    \pgfpathmoveto{\pgfpoint{0}{-\pgf@ya}}
    \pgfpathcurveto{\pgfpoint{\pgf@xc}{-\pgf@yc}}
    {\pgfpoint{\pgf@xc}{\pgf@yc}}{\pgfpoint{\pgf@xa}{\pgf@ya}}

    % Todo: get rid of this repition, somehow ya gets overwritten by the
    % above path
    \semimajor \pgf@xa =\pgf@x \pgf@ya = \pgf@y
    \semiminor \pgf@xb = \pgf@x \pgf@yb = \pgf@y

    % Calculate x and y coordinates of support for bezier curve
    \pgf@xc = \pgf@xb \advance \pgf@xc by 0.1\pgf@xb
    \pgf@yc = 0.5\pgf@ya

    % Draw second half of lens
    \pgfpathcurveto{\pgfpoint{-\pgf@xc}{\pgf@yc}}
    {\pgfpoint{-\pgf@xc}{-\pgf@yc}}{\pgfpoint{0}{-\pgf@ya}}
    \pgfpathclose
  }
}


% Horizontal optical elements are horizontal on paper (i.e. a horizontal
% waveplate), that is the beam passes vertically through it


% Cross optical elements are ones through which the beam may pass both
% horizontally and vertically

% Beamsplitter
% Todo respect minimum width
\pgfdeclareshape{beam splitter}{%
  \savedanchor{\southwest}{%
    \optsetxandyvecbyvalueofkey{/tikz/beam splitter width} \pgfpointxy{-0.5}{-0.5}}
  \savedanchor{\northeast}{%
    \optsetxandyvecbyvalueofkey{/tikz/beam splitter width} \pgfpointxy{0.5}{0.5}}
  \savedanchor{\beamnee}{%
    \optsetxandyvecbyvalueofkey{/tikz/beam splitter width} \pgfpointxy{0.5}{0.5}
    \pgf@xa = \pgf@x 
    \pgfpointorigin
    \pgf@ya = \pgf@y \advance\pgf@ya by \pgfkeysvalueof{/tikz/waist}
    \pgfpoint{\pgf@xa}{\pgf@ya}}
  
  \inheritanchor[from=vertical optical element]{north}
  \inheritanchor[from=vertical optical element]{north west}
  \inheritanchor[from=vertical optical element]{west}
  \inheritanchor[from=vertical optical element]{south west}
  \inheritanchor[from=vertical optical element]{south}
  \inheritanchor[from=vertical optical element]{south east}
  \inheritanchor[from=vertical optical element]{east}
  \inheritanchor[from=vertical optical element]{north east}
  \inheritanchor[from=vertical optical element]{center}
  
  % Define anchors where the beam hits variaus parts of the cube
  \anchor{beam nee}{%
    \beamnee
  }
  
  \anchor{beam nne}{%
    \northeast \pgf@ya=\pgf@y
    \beamnee \pgf@yc = \pgf@y
    \pgfpointorigin
    \pgf@xa = \pgf@x \advance\pgf@xa by \pgf@yc
    \pgfpoint{\pgf@xa}{\pgf@ya}}
  
  \anchor{beam nnw}{%
    \southwest \pgf@xa=\pgf@x
    \beamnee \pgf@yc = \pgf@y
    \pgfpointorigin
    \pgf@ya = \pgf@y \advance\pgf@ya by \pgf@yc
    \pgfpoint{\pgf@xa}{\pgf@ya}}

  \anchor{beam nww}{%
    \southwest \pgf@xa=\pgf@x
    \beamnee \pgf@yc = \pgf@y
    \pgfpointorigin
    \pgf@ya = \pgf@y \advance\pgf@ya by \pgf@yc
    \pgfpoint{\pgf@xa}{\pgf@ya}}

  \anchor{beam sww}{%
    \southwest \pgf@xa=\pgf@x
    \beamnee \pgf@yc = \pgf@y
    \pgfpointorigin
    \pgf@ya = \pgf@y \advance\pgf@ya by -\pgf@yc
    \pgfpoint{\pgf@xa}{\pgf@ya}}

  \anchor{beam ssw}{%
    \southwest \pgf@ya=\pgf@y
    \beamnee \pgf@yc = \pgf@y
    \pgfpointorigin
    \pgf@xa = \pgf@x \advance\pgf@xa by -\pgf@yc
    \pgfpoint{\pgf@xa}{\pgf@ya}}

  \anchor{beam sse}{%
    \southwest \pgf@ya=\pgf@y
    \beamnee \pgf@yc = \pgf@y
    \pgfpointorigin
    \pgf@xa = \pgf@x \advance\pgf@xa by \pgf@yc
    \pgfpoint{\pgf@xa}{\pgf@ya}}

  \anchor{beam see}{%
    \northeast \pgf@xa=\pgf@x
    \beamnee \pgf@yc = \pgf@y
    \pgfpointorigin
    \pgf@ya = \pgf@y \advance\pgf@ya by -\pgf@yc
    \pgfpoint{\pgf@xa}{\pgf@ya}}


  \backgroundpath{%
    % store lower left in xa/ya and upper right in xb/yb 
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y 
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y

    % No rounded corners (don't know how to connect
    % diagonal to rounded corners directly
    \pgfsetcornersarced{\pgfpointorigin}
    
    % Draw a diagonal line
    \ifnum \pgfkeysvalueof{/tikz/flip beam splitter axis} = 1
    \pgfpathmoveto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
    \else
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \fi
    \pgfpathclose


    % Draw cube
    \pgfpathmoveto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathclose
  }

}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "optikztest"
%%% End: 

